Constructing stable de Sitter in M-theory from higher curvature corrections

We consider dimensional reductions of M-theory on $\mathbb{T}^{7}/\mathbb{Z}_{2}^{3}$ with the inclusion of arbitrary metric flux and spacetime filling KK monopoles. With these ingredients at hand, we are able to construct a novel family of non-supersymmetric yet tachyon free Minkowski extrema. These solutions are supported by pure geometry with no extra need for gauge fluxes and possess a fully stable perturbative mass spectrum, up to a single flat direction. Such a direction corresponds to the overall internal volume, with respect to which the scalar potential exhibits a no-scale behavior. We then provide a mechanism that lifts the flat direction to give it a positive squared mass while turning Mkw$_{4}$ into dS$_{4}$. The construction makes use of the combined effect of $G_{7}$ flux and higher curvature corrections. Our solution is scale separated and the quantum corrections are small. Finally we speculate on novel possibilities when it comes to scale hierarchies within a given construction of this type, and possible issues with the choice of quantum vacuum.

==> conclusion.tex <==
\section{Conclusion and discussion}
\label{sec:conclusion}
